Viral Lattice Theory: A Biophysical Framework for Collective Virion Motion

Viral Lattice Theory develops a testable framework for collective motion and mechanical response of virions and virus-like particles (VLPs) in viscoelastic environments. Its central problem is observational ambiguity: distinct interparticle forces, material relaxation processes, and hydrodynamic couplings can produce similar particle trajectories or equilibrium measurements. We ask which additional measurements can distinguish these mechanisms. Combining lattice dynamics, stochastic mechanics, and linear response theory, the framework derives memory-dependent forces and, under thermal-equilibrium assumptions, fluctuation-dissipation-consistent noise. Explicit observation models account for finite camera exposure and support parameter-identifiability tests and experimental design. In a synthetic response-fluctuation benchmark, models with matching equilibrium covariance and nearly matching response magnitude differ by approximately 28 degrees in response phase and 40% in spectral density at a selected crossover, demonstrating the discriminating value of complementary observables. A crystal-response example uses satellite tobacco mosaic virus geometry and published acoustic summaries to calibrate a spectral peak and test a separately reserved linewidth. An HPV-inspired VLP model extends the framework to classical stochastic transport between intact, reversibly deformed, and damaged structural states, illustrating recovery and delayed damage after delivery. Path-survival and driven-cycle calculations distinguish transient loading from sustained nonequilibrium behavior. A separate viral-phonon quantization postulate is presented as a conditional quantum extension, not an established biological effect. The results provide synthetic and conditional comparisons that specify experimentally testable distinctions.

==> vlt-graphics.tex <==
\makeatletter
\newcommand{\vlB}[1]{#1}
\newcommand{\vlSeg}[6]{\vlStroke{#1}{#2}{#3}{#4}{#5}{#6}}
\newcommand{\vlRect}[4]{\put(#1,#2){\rule{#3pt}{#4pt}}}
\def\vSa#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.750000}{0.375000}}
\def\vSb#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.050000}{0.525000}}
\def\vSc#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.000000}{0.500000}}
\def\vSd#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.650000}{0.325000}}
\def\vSe#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.100000}{0.550000}}
\def\vSf#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.900000}{0.450000}}
\def\vSg#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.700000}{0.850000}}
\def\vSh#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.550000}{0.275000}}
\def\vSi#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.400000}{0.700000}}
\def\vSj#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.350000}{0.675000}}
\def\vSk#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.800000}{0.400000}}
\def\vSl#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.500000}{0.250000}}
\def\vSm#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.400000}{0.200000}}
\def\vSn#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.850000}{0.425000}}
\def\vSo#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.500000}{0.750000}}
\def\vSp#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.600000}{0.800000}}
\def\vSq#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.300000}{0.650000}}
\def\vSr#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.700000}{0.350000}}
\def\vSs#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.150000}{0.575000}}
\def\vSt#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.900000}{0.950000}}
\def\vSu#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.600000}{0.300000}}
\def\vSv#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.800000}{0.900000}}
\def\vSw#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.450000}{0.725000}}
\def\vSx#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.200000}{0.600000}}
\def\vSy#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{2.200000}{1.100000}}
\def\vSz#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.950000}{0.475000}}
\def\vSaa#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.250000}{0.625000}}
\def\vSab#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{2.000000}{1.000000}}
\def\vSac#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.780000}{0.390000}}
\def\vSad#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.650000}{0.825000}}
\def\vSae#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{2.100000}{1.050000}}
\def\vSaf#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{2.800000}{1.400000}}
\def\vSag#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.750000}{0.875000}}
\def\vSah#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.550000}{0.775000}}
\def\vSai#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.850000}{0.925000}}
\def\vSaj#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.540000}{0.270000}}
\def\vSak#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.510000}{0.255000}}
\def\vSal#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.570000}{0.285000}}
\def\vSam#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.55}{0.275}}
\def\vSan#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.35}{0.175}}
\def\vSao#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.7}{0.35}}
\def\vSap#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.232}{0.616}}
\def\vSaq#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.85}{0.425}}
\def\vSar#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.344}{0.672}}
\def\vSas#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.12}{0.56}}
\def\vSat#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{28}{14}}
\def\vSau#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{16}{8}}
\def\vSav#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{19}{9.5}}
\def\vSaw#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.45}{0.225}}
\def\vSax#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.4}{0.7}}
\def\vSay#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.896}{0.448}}
\def\vSaz#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.3}{0.65}}
\def\vSba#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.65}{0.325}}
\def\vSbb#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1}{0.5}}
\def\vSbc#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{2}{1}}
\def\vSbd#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.6}{0.3}}
\def\vSbe#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.4}{0.2}}
\def\vSbf#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.5}{0.25}}
\def\vSbg#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.2}{0.6}}
\def\vSbh#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.8}{0.4}}
\def\vSbi#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.1}{0.55}}
\def\vSbj#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.9}{0.45}}
\def\vSbk#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.5}{0.75}}
\def\vSbl#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{2.400000}{1.200000}}
\def\vSbm#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.952}{0.476}}
\def\vSbn#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.75}{0.375}}
\def\vSbo#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.365685}{0.682843}}
\def\vSbp#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.492820}{0.746410}}
\def\vSbq#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.450000}{0.225000}}
\def\vSbr#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{0.820000}{0.410000}}
\def\vSbs#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.120000}{0.560000}}
\def\vSbt#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.7}{0.85}}
\def\vSbu#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.288}{0.644}}
\def\vSbv#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{2.500000}{1.250000}}
\def\vSbw#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{1.15}{0.575}}
\def\vSbx#1#2#3#4{\vlSeg{#1}{#2}{#3}{#4}{3.000000}{1.500000}}
\def\vRa#1#2#3{\vlRect{#1}{#2}{#3}{0.460000}}
\def\vRb#1#2#3{\vlRect{#1}{#2}{#3}{27.100000}}
\def\vRc#1#2#3{\vlRect{#1}{#2}{#3}{14.00000}}
\def\vRd#1#2#3{\vlRect{#1}{#2}{#3}{3.08263}}
\def\vRe#1#2#3{\vlRect{#1}{#2}{#3}{2.93000}}
\def\vRf#1#2#3{\vlRect{#1}{#2}{#3}{139.00000}}
\def\vRg#1#2#3{\vlRect{#1}{#2}{#3}{4.33556}}
\def\vRh#1#2#3{\vlRect{#1}{#2}{#3}{2.61333}}
\makeatother

